Recovery of transversely-isotropic elastic material parameters in induction motor rotors

We propose numerical algorithms for recovering parameters in eigenvalue problems for linear elasticity of transversely isotropic materials. Specifically, the algorithms are used to recover the elastic constants of a rotor core. Numerical tests show that in the noiseless setup, two pairs of bending modes are sufficient for recovering one to four parameters accurately. To recover all five parameters that govern the elastic properties of electric engines accurately, we require three pairs of bending modes and one torsional mode. Moreover, we study the stability of the inversion method against multiplicative noise; for tests in which the data contained multiplicative noise of at most $1\%$, we find that all parameters can be recovered with an error less than $10\%$.

==> Application_measured_data.tex <==
\section{Measured data} \label{sec:measured}
In this section, we discuss some details about the measured eigenfrequencies. For the model considered in this paper, there are two main types of eigenmodes: bending modes and torsional modes. Bending modes usually affect the shafts (see Figure \ref{fig.rotor_modes}, left) and can be measured quite accurately. On the other hand, torsional modes mostly affect the central region where the rotor core and the rings and bars are located (see Figure \ref{fig.rotor_modes}, right). Due to the mismatch between the experimental setup and the mathematical model (eigenvalue problem) discussed in Section \ref{sec:setup_and_model}, the measured torsional modes are significantly different from the numerically calculated torsional modes, and cannot be used to recover useful data. The damping of the torsional mode also changes the order of the eigenfrequencies. That is, instead of having two pairs of bending modes before observing the torsional mode, we may observe only one pair of bending modes  before observing the torsional mode. This becomes an issue in the cost functions we minimize in \eqref{eq:minimisation_exact} and \eqref{eq:minimisation_approx}, as the order of the eigenfrequencies are important. For the tests performed in this section, we match the numerical eigenfrequencies corresponding to bending modes to the measured bending modes.  



Figure shows the results obtained via EKI and the least squares approach. Here, we see that both the least squares and EKI methods recover essentially the same value for the shear modulus. On the other hand, the results for the Young's modulus are not in agreement, indicating that either a better mathematical model or more data would be needed in order to have a more confident estimate of the Young's modulus.

==> inverse_prob.tex <==
\section{Inverse eigenvalue problem} \label{sec:inv_problem}
In this section, we state the inverse eigenvalue problem for the material parameters $\mathbf{p} \in \R ^5$, and propose some methods for recovering the said parameters. Suppose that a measuring procedure recovers a set of eigenvalues $\Lambda_1,\dots,\Lambda_N$ for the eigenvalue problem \eqref{eq:eigenvalue_problem}. 
% Suppose further that data about the values of the corresponding eigenfunctions $\varphi_1,\dots \varphi_N$ at certain points $\x_1,\dots, \x_k$ of the domain are also available. 
Our aim is then to recover the parameters $\mathbf{p} = [E_p, E_z, G_p, G_{zp}, \nu_{pz}]$ from these data. We denote by $f:\R^5\rightarrow\R^N$ the mapping from $\mathbf{p}$ to the first $N$ natural eigenvalues $\Lambda_1,\dots, \Lambda_N$. 
% and $g:\R^5 \rightarrow \R^{k\times N}$ the mapping from $\mathbf{p}$ to the (normalized) values of the eigenfunctions $\varphi_1,\dots, \varphi_N$ corresponding to the eigenvalues $\Lambda_1, \dots, \Lambda_N$ at $\x_1,\dots,\x_k$. Of course, $k$ depends on some practical matters, such as the number of sensors available, and the number of measurements that will be made. 
In order to recover the parameter $\mathbf{p}$, we aim to minimize a cost function which relates the measured data with the output of the map $f$.

\subsection{Measurements without noise}
We start by considering an inverse problem under the assumptions that the measurements do not contain noise. For linear elasticity eigenvalue problems, we aim to find $\mathbf{p}$ such that 

\begin{equation}\label{eq:minimisation_exact}
    \min_{\mathbf{p}\in\R} \norm{f(\mathbf{p})-\bm{\lambda}}{\ell^2}^2.
\end{equation}
% \begin{equation}\label{eq:minimisation_exact}
%     \min_{\mathbf{p}\in\R} \norm{f(\mathbf{p})-\bm{\lambda}}{\ell^2}^2 + \norm{g(\mathbf{p})-\bm{\varphi}}{\ell ^2}^2.
% \end{equation}

That is, we fit, in the least squares sense, the measured eigenvalues with the computed eigenvalues via the mapping $f$. This problem may be solved via iterative methods. In particular, we employ the minimizers from Python's \code{SciPy} package. The input required by the algorithms is an initial guess for the parameter(s). Here, we use Hessian-based methods, such as the BFGS-B or L-BFGS-B \cite{BLNZ95-LBFGS,ZBLN97-LBFGSB}, or the sequential least squares (SLSQP) \cite{K88-SQP} for solving the minimisation problem. 

We now perform a numerical test for a scenario where the first 6 natural eigenvalues are given, without noise, for the true parameters $\mathbf{p}_{\mathrm{true}} = [2e11,2e8,7.69e10,5e8,0.3]$, where the units of the Young's and shear moduli are given in Pascals. Table shows that it is possible to recover single or multiple parameters (excluding the Poisson ratio) with a relative error of magnitude 1e-6 or less, provided that the mathematical model captures the experimental model exactly, and that there is no noise in the measurements. We note however that the measurements cannot be exact, so we need to consider models for the noise in measurement.

\subsection{Multiplicative noise}
In this section, we consider the case for which we assume that the measurements come with multiplicative noise. That is, each entry of the measurement $\bm\lambda^\delta$ is given by $\lambda_i ^\delta = (1+p_i) \lambda_i$, where $p_i$ is drawn from a normal distribution $N(0, \delta^2)$ with mean $0$ and variance $\delta^2$. This means that  $\lambda_i^\delta  \sim N(\lambda_i, \lambda_i ^ 2 \delta ^2)$. 

In order to deal with measurement with noise, we may solve instead of \eqref{eq:minimisation_exact} the minimization problem 

\begin{equation}\label{eq:minimisation_approx}
    \min_{p\in\R} \sum_{i=1}^N \frac{(f(p)_i - \lambda_i^\delta)^2}{f(p)_i^2 \delta ^2} + \log(f(p)_i),
\end{equation}
which corresponds to a maximum likelihood estimator for $\mathbf{p}$. On the other hand,  


In order to assess the magnitude of allowable noise for which we still recover sensible data, we now consider the following increasing noise levels: $\delta = 0.0001, 0.0005, 0.001$. From our numerical tests, we observe that starting from $\delta= 0.001$, the parameters recovered by the algorithm already have a relative error which is  $10\%$ or larger.

\subsection{Measured data}
In this section, we discuss some details about the measured eigenfrequencies. For the model considered in this paper, there are two main types of eigenmodes: bending modes and torsional modes. Bending modes usually affect the shafts (see Figure \ref{fig.rotor_modes}, left) and can be measured quite accurately. On the other hand, torsional modes mostly affect the central region where the rotor core and the rings and bars are located (see Figure \ref{fig.rotor_modes}, right). Due to the experimental setup discussed in Section \ref{sec:setup_and_model} where the rotor is laid at rest on a rubber block, the measured torsional modes are significantly damped, and cannot be used to recover useful data. The damping of the torsional mode also changes the order of the eigenfrequencies. That is, instead of having two pairs of bending modes before observing the torsional mode, we may observe only one pair of bending modes  before observing the torsional mode. This becomes an issue in the cost functions we minimize in \eqref{eq:minimisation_exact} and \eqref{eq:minimisation_approx}, as the order of the eigenfrequencies are important. In this work, we base the order of the eigenfrequencies on the measured data.  

\begin{figure}[h!]
	\begin{tabular}{cc}
		\includegraphics[width=0.45\linewidth]{images/bending_mode.png} &
		\includegraphics[width=0.45\linewidth]{images/torsional_mode.png} 
	\end{tabular}
	\caption{Illustration of mode types. Left: bending mode, Right: torsional mode} \label{fig.rotor_modes}
\end{figure}
\subsection{Eigenfunction measurements}

One way to improve the parameter estimation in the presence of noise is to add the eigenfunction measurements to the cost function considered in \eqref{eq:minimisation_approx}. To this end, we need to suggest a method for choosing the locations of the sensors, depending on the parameters that need to be recovered. For instance, if we aim to recover $E_z$, we perform the forward map for several values of $E_z$, and take note of the displacement magnitudes in the boundary of the domain. Following this, we measure, for each point, the standard deviation of the displacement magnitude. This gives an indication of the locations for which the change in the displacement magnitude are the most sensitive with respect to the change in the parameter. Another alternative for choosing the locations involve measuring the points for which the average displacement magnitude over all parameter values is maximum. We present in Figure \ref{fig.rotor_withsens} an illustration, where the red and blue points indicate the locations with maximum standard deviation and maximum average displacement, respectively. 


\begin{figure}[h!]\centering
	\includegraphics[width=0.5\linewidth]{rotor_with_sensorlocs.png} 
	\caption{Sample image of ideal sensor locations on a rotor.} \label{fig.rotor_withsens}
\end{figure}


% the relative errors in the recovered parameter can reach the scale of $10 \delta$, and hence for $\delta = 0.01$ the recovered parameter is already very far away from the real data. To further understand this, we calculate $\bm{\lambda}$ and $\bm{\varphi}$ from a reference value $E_z^*$, and consider perturbations $\bm{\lambda}^\delta, \bm{\varphi}^\delta$ of these calculated values to see the effect on the target functions $\norm{f(p)-\bm{\lambda}^\delta}{\ell^2}^2$ and $\norm{g(p)-\bm{\varphi}^\delta}{\ell ^2}^2$.

%  As a starting point, we consider a linear map 

% \begin{equation}\label{eq:lin_map}
% f(x) = Ax+\mathbf{b}.
% \end{equation}

% Since the parameter $E_z$ is a scalar, our matrix $A$ is actually a $N\times 1$ vector. We then deduce the entries of $A$ and $\mathbf{b}$ by the method of least-squares. 

% Following this, we then add some noise $\delta w$ to $\lambda_i$ and try to find $x_\delta$ corresponding to the perturbed $\lambda$s. A simple choice for computing $x_\delta$ involves solving the least-norm solution of \eqref{eq:lin_map}. This allows us to deduce a threshold for the noise level $\delta$.  For the linear approximation \eqref{eq:lin_map} resulting from data which are within $5\%$ of the correct value, we found that taking $\delta = p/100$ leads to an error of approximately $2p^2/100$ in approximating the unknown parameter $E_z$.
